On Controlling Knockout Tournaments Without Perfect Information

Over the last decade, extensive research has been conducted on the algorithmic aspects of designing single-elimination (SE) tournaments. Addressing natural questions of algorithmic tractability, we identify key properties of input instances that enable the tournament designer to efficiently schedule the tournament in a way that maximizes the chances of a preferred player winning. Much of the prior algorithmic work on this topic focuses on the perfect (complete and deterministic) information scenario, especially in the context of fixed-parameter algorithm design. Our contributions constitute the first fixed-parameter tractability results applicable to more general settings of SE tournament design with potential imperfect information.

==> gtmacros.tex <==
% Game Theory Macros

% General maths stuff
\renewcommand{\phi}{\varphi}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

% general
\newcommand{\prof}[1]{\boldsymbol{#1}}
\newcommand{\cprod}[1]{\boldsymbol{#1}}
\newcommand{\pref}{\succ}
\newcommand{\prefeq}{\succeq}
\newcommand{\dispref}{\prec}
\newcommand{\disprefeq}{\preceq}
\newcommand{\indiff}{\sim}

% coalitional games
\newcommand{\mc}{\Delta}
\newcommand{\mcseq}{\vec{\Delta}}

% extensive-form games
%\newcommand{\turn}{\rho}
%\newcommand{\actions}{\chi}
% \newcommand{\turn}{\underline{i}}
\newcommand{\actions}{\underline{A}}
\newcommand{\successor}{\sigma}
\newcommand{\outcome}{\text{\rm out}}

% normal-form games
\usepackage{readarray}
\definecolor{darkred}{rgb}{0.64,0,0}
\definecolor{darkcyan}{rgb}{0,0.55,0.55}
\newcommand{\rowcolor}[1]{\textcolor{black}{#1}}
\newcommand{\columncolor}[1]{\textcolor{black}{#1}}

\newcommand{\nfgame}[1]{%
\getargsC{#1}
\begin{tikzpicture}[scale=0.5]
\node (RT) at (-2,1) [label=left:\rowcolor{\argi}] {};
\node (RB) at (-2,-1) [label=left:\rowcolor{\argii}] {};
\node (CL) at (-1,2) [label=above:\columncolor{\argiii}] {};
\node (CR) at (1,2) [label=above:\columncolor{\argiv}] {};
\node (RTL) at (-1.4,0.6) {\rowcolor{\argv}}; % top/left row player payoff
\node (CTL) at (-0.6,1.4) {\columncolor{\argvi}}; % top/left column player payoff
\node (RBL) at (-1.4,-1.4) {\rowcolor{\argvii}};
\node (CBL) at (-0.6,-0.6) {\columncolor{\argviii}};
\node (RTR) at (0.6,0.6) {\rowcolor{\argix}};
\node (CTR) at (1.4,1.4) {\columncolor{\argx}};
\node (RBR) at (0.6,-1.4) {\rowcolor{\argxi}};
\node (CBR) at (1.4,-0.6) {\columncolor{\argxii}};
\draw[-,very thick] (-2,-2) to (2,-2);
\draw[-,very thick] (-2,0) to (2,0);
\draw[-,very thick] (-2,2) to (2,2);
\draw[-,very thick] (-2,-2) to (-2,2);
\draw[-,very thick] (0,-2) to (0,2);
\draw[-,very thick] (2,-2) to (2,2);
\draw[-,very thin] (-2,2) to (0,0);
\draw[-,very thin] (0,0) to (2,-2);
\draw[-,very thin] (-2,0) to (0,-2);
\draw[-,very thin] (0,2) to (2,0);
\end{tikzpicture}}

%\nfgamethree{T C B L M R 1 2 3 4 5 6 7 8 9 10 11 12 13 14 15 16 17 18}
\newcommand{\nfgamethree}[1]{%
\getargsC{#1}
\begin{tikzpicture}[scale=0.65]
\node (RT) at (-3,2)  [label=left:\rowcolor{\argi}] {};
\node (RC) at (-3,0)  [label=left:\rowcolor{\argii}] {};
\node (RB) at (-3,-2) [label=left:\rowcolor{\argiii}] {};
\node (CL) at (-2,3)  [label=above:\columncolor{\argiv}] {};
\node (CM) at (0,3)   [label=above:\columncolor{\argv}] {};
\node (CR) at (2,3)   [label=above:\columncolor{\argvi}] {};

\node (RTL) at (-2.4,1.6) {\rowcolor{\argvii}}; 
\node (CTL) at (-1.6,2.4) {\columncolor{\argviii}};
\node (RCL) at (-2.4,-0.4) {\rowcolor{\argix}}; 
\node (CCL) at (-1.6,0.4) {\columncolor{\argx}};
\node (RBL) at (-2.4,-2.4) {\rowcolor{\argxi}};
\node (CBL) at (-1.6,-1.6) {\columncolor{\argxii}};

\node (RTM) at (-0.4,1.6) {\rowcolor{\argxiii}}; 
\node (CTM) at (0.4,2.4) {\columncolor{\argxiv}};
\node (RCM) at (-0.4,-0.4) {\rowcolor{\argxv}}; 
\node (CCM) at (0.4,0.4) {\columncolor{\argxvi}};
\node (RBM) at (-0.4,-2.4) {\rowcolor{\argxvii}};
\node (CBM) at (0.4,-1.6) {\columncolor{\argxviii}};

\node (RTR) at (1.6,1.6) {\rowcolor{\argxix}}; 
\node (CTR) at (2.4,2.4) {\columncolor{\argxx}};
\node (RCR) at (1.6,-0.4) {\rowcolor{\argxxi}}; 
\node (CCR) at (2.4,0.4) {\columncolor{\argxxii}};
\node (RBR) at (1.6,-2.4) {\rowcolor{\argxxiii}};
\node (CBR) at (2.4,-1.6) {\columncolor{\argxxiv}};

\draw[-,very thick] (-3,-3) to (3,-3);
\draw[-,very thick] (-3,-1) to (3,-1);
\draw[-,very thick] (-3,1) to (3,1);
\draw[-,very thick] (-3,3) to (3,3);
\draw[-,very thick] (-3,-3) to (-3,3);
\draw[-,very thick] (-1,-3) to (-1,3);
\draw[-,very thick] (1,-3) to (1,3);
\draw[-,very thick] (3,-3) to (3,3);
\draw[-,very thin] (-3,3) to (3,-3);
\draw[-,very thin] (-1,3) to (3,-1);
\draw[-,very thin] (-3,1) to (1,-3);
\draw[-,very thin] (1,3) to (3,1);
\draw[-,very thin] (-3,-1) to (-1,-3);
\end{tikzpicture}}

%\nfgametwothree{T B L M R 1 2 3 4 5 6 7 8 9 10 11 12}
\newcommand{\nfgametwothree}[1]{%
\getargsC{#1}
\begin{tikzpicture}[scale=0.65]
\node (RT) at (-3,1)  [label=left:\rowcolor{\argi}] {};
\node (RB) at (-3,-1) [label=left:\rowcolor{\argii}] {};
\node (CL) at (-2,2)  [label=above:\columncolor{\argiii}] {};
\node (CM) at (0,2)  [label=above:\columncolor{\argiv}] {};
\node (CR) at (2,2)  [label=above:\columncolor{\argv}] {};

\node (RTL) at (-2.4,0.6) {\rowcolor{\argvi}}; 
\node (CTL) at (-1.6,1.4) {\columncolor{\argvii}};
\node (RBL) at (-2.4,-1.4) {\rowcolor{\argxii}};
\node (CBL) at (-1.6,-0.6) {\columncolor{\argxiii}};

\node (RTM) at (-0.4,0.6) {\rowcolor{\argviii}}; 
\node (CTM) at (0.4,1.4) {\columncolor{\argix}};
\node (RBM) at (-0.4,-1.4) {\rowcolor{\argxiv}};
\node (CBM) at (0.4,-0.6) {\columncolor{\argxv}};

\node (RTR) at (1.6,0.6) {\rowcolor{\argx}}; 
\node (CTR) at (2.4,1.4) {\columncolor{\argxi}};
\node (RBR) at (1.6,-1.4) {\rowcolor{\argxvi}};
\node (CBR) at (2.4,-0.6) {\columncolor{\argxvii}};

\draw[-,very thick] (-3,-2) to (3,-2);
\draw[-,very thick] (-3,0) to (3,0);
\draw[-,very thick] (-3,2) to (3,2);
\draw[-,very thick] (-3,-2) to (-3,2);
\draw[-,very thick] (-1,-2) to (-1,2);
\draw[-,very thick] (1,-2) to (1,2);
\draw[-,very thick] (3,-2) to (3,2);
\draw[-,very thin] (-3,2) to (1,-2);
\draw[-,very thin] (-1,2) to (3,-2);
\draw[-,very thin] (-3,0) to (-1,-2);
\draw[-,very thin] (1,2) to (3,0);
\draw[-,very thin] (-3,-2) to (-1,-2);
\end{tikzpicture}}

